Uncertainty Surrogates for Deep Learning

In this paper we introduce a novel way of estimating prediction uncertainty in deep networks through the use of uncertainty surrogates. These surrogates are features of the penultimate layer of a deep network that are forced to match predefined patterns. The patterns themselves can be, among other possibilities, a known visual symbol. We show how our approach can be used for estimating uncertainty in prediction and out-of-distribution detection. Additionally, the surrogates allow for interpretability of the ability of the deep network to learn and at the same time lend robustness against adversarial attacks. Despite its simplicity, our approach is superior to the state-of-the-art approaches on standard metrics as well as computational efficiency and ease of implementation. A wide range of experiments are performed on standard datasets to prove the efficacy of our approach.

==> latex/21_fig_teaser.tex <==
\newcommand{\colwidth}{0.24\linewidth}
\newcommand{\gap}{@{\hspace{0.5mm}}}

\begin{figure}
\centering
\begin{tabular}{c\gap c\gap c\gap c\gap}
\includegraphics[width=\colwidth]{./images/teaser/splits/31_green_car_13054702.png}&
\includegraphics[width=\colwidth]{./images/teaser/splits/59_green_frog_25773603.png}&
\includegraphics[width=\colwidth]{./images/teaser/splits/95_red_bird_4394087.png}&
\includegraphics[width=\colwidth]{./images/teaser/splits/35_red_bird_16191183.png}\\
% \vspace{-1em}
0.1305 & 0.2577 & 0.4394 & 0.1619\\
& & & \\
\end{tabular}
\caption{Example output of uncertainty surrogates when trained with 10 text images of the class names. The rows from top contain: the original images from the CIFAR10 dataset~\cite{}, our uncertainty surrogates, the pattern corresponding to the predicted label, the pattern corresponding to the true label, the uncertainty score as a colored bar (green for correctly predicted and red for incorrectly predicted examples), and the numerical value of the uncertainty score. The four columns show the follwoing different cases of prediction from left to right: low uncertainty and correct, high uncertainty but correct, high uncertainty and wrong, low uncertainty and wrong. Apart from this last case, the uncertainty computed through our prediction surrogates is a good indicator of the quality of the decision.}
\label{fig:teaser}
\end{figure}

==> latex/22_fig_cifar10words.tex <==
\renewcommand{\colwidth}{0.08\linewidth}
\renewcommand{\gap}{@{\hspace{0.5mm}}}

\begin{figure*}
\centering
\begin{tabular}{c\gap c\gap c\gap c\gap c\gap c\gap c\gap c\gap c\gap c\gap c\gap c\gap}

\includegraphics[width=\colwidth]{./images/splits_cifar10words/95_green_car_13451861.png}&
\includegraphics[width=\colwidth]{./images/splits_cifar10words/92_green_dog_1465128.png}&
\includegraphics[width=\colwidth]{./images/splits_cifar10words/98_green_plane_1948236.png}&
\includegraphics[width=\colwidth]{./images/splits_cifar10words/99_green_cat_11086719.png}&

\includegraphics[width=\colwidth]{./images/splits_cifar10words/44_green_plane_3222305.png}&
\includegraphics[width=\colwidth]{./images/splits_cifar10words/95_green_truck_29344362.png}&
\includegraphics[width=\colwidth]{./images/splits_cifar10words/00_green_bird_23467687.png}&
\includegraphics[width=\colwidth]{./images/splits_cifar10words/00_green_truck_29432157.png}&

\includegraphics[width=\colwidth]{./images/splits_cifar10words/05_red_cat_32756782.png}&
\includegraphics[width=\colwidth]{./images/splits_cifar10words/10_red_ship_34134647.png}&
\includegraphics[width=\colwidth]{./images/splits_cifar10words/26_red_dog_32670072.png}&
\includegraphics[width=\colwidth]{./images/splits_cifar10words/02_red_bird_34826124.png}\\


% \includegraphics[width=\colwidth]{./images/splits_cifar10words/09_red_truck_21100867.png}

% \vspace{-1em} 
% 0.1305 & 0.2577 & 0.4394 & 0.1619\\
0.1345 & 0.1465 & 0.1948 & 0.1108 & 0.3222 & 0.2934 & 0.2346 & 0.2943 & 0.3275 & 0.3413 & 0.3267 & 0.3482\\
& & & & & & & & & & & \\
\end{tabular}
\caption{Example output of uncertainty surrogates when trained with 10 text images of the class names. The rows from top contain: the original images from the CIFAR10 dataset~\cite{}, our uncertainty surrogates, the pattern corresponding to the predicted label, the pattern corresponding to the true label, the uncertainty score as a colored bar (green for correctly predicted and red for incorrectly predicted examples), and the numerical value of the uncertainty score.}
\label{fig:cifar10words}
\end{figure*}

==> latex/23_fig_mnist_strip.tex <==
\renewcommand{\colwidth}{ 0.045 \linewidth}
\renewcommand{\gap}{@{\hspace{0.5mm}}}

\begin{figure*}
\centering

\begin{tabular}{c\gap c\gap c\gap c\gap c\gap c\gap c\gap c\gap c\gap c\gap c\gap c\gap c\gap c\gap c\gap c\gap c\gap c\gap c\gap c\gap}
\includegraphics[width=\colwidth]{./images/splits_mnist_digits/70_green_horse_09362455.png}&
\includegraphics[width=\colwidth]{./images/splits_mnist_digits/05_green_car_0966025.png}&
\includegraphics[width=\colwidth]{./images/splits_mnist_digits/67_green_bird_117122136.png}&
\includegraphics[width=\colwidth]{./images/splits_mnist_digits/65_green_deer_11872817.png}&
\includegraphics[width=\colwidth]{./images/splits_mnist_digits/76_green_cat_12104888.png}&
\includegraphics[width=\colwidth]{./images/splits_mnist_digits/91_green_ship_14096366.png}&
\includegraphics[width=\colwidth]{./images/splits_mnist_digits/42_green_ship_14098191.png}&
\includegraphics[width=\colwidth]{./images/splits_mnist_digits/35_green_ship_1415014.png}&
\includegraphics[width=\colwidth]{./images/splits_mnist_digits/62_green_truck_14182585.png}&
\includegraphics[width=\colwidth]{./images/splits_mnist_digits/84_green_ship_14208893.png}&
\includegraphics[width=\colwidth]{./images/splits_mnist_digits/59_green_truck_14249483.png}&
\includegraphics[width=\colwidth]{./images/splits_mnist_digits/49_green_cat_14500806.png}&
\includegraphics[width=\colwidth]{./images/splits_mnist_digits/12_green_dog_14644496.png}&
\includegraphics[width=\colwidth]{./images/splits_mnist_digits/21_green_bird_14795314.png}&
\includegraphics[width=\colwidth]{./images/splits_mnist_digits/40_green_dog_14876646.png}&
\includegraphics[width=\colwidth]{./images/splits_mnist_digits/36_green_truck_15184802.png}&
\includegraphics[width=\colwidth]{./images/splits_mnist_digits/47_green_deer_16087078.png}&
\includegraphics[width=\colwidth]{./images/splits_mnist_digits/90_green_ship_18634838.png}&
\includegraphics[width=\colwidth]{./images/splits_mnist_digits/15_green_deer_20723826.png}&
\includegraphics[width=\colwidth]{./images/splits_mnist_digits/45_red_frog_14070812.png}\\

0.094 &
0.097 &
0.117 &
0.119 &
0.121 &
0.141 &
0.141 &
0.142 &
0.142 &
0.142 &
0.142 &
0.145 &
0.146 &
0.148 &
0.149 &
0.152 &
0.161 &
0.186 &
0.207 &
0.141 \\

\end{tabular}
\caption{}
\label{}
\end{figure*}

==> latex/24_fig_fashion_strip.tex <==
\renewcommand{\colwidth}{ 0.060000000000000005 \linewidth}
\renewcommand{\gap}{@{\hspace{0.5mm}}}

\begin{figure*}
\centering

\begin{tabular}{c\gap c\gap c\gap c\gap c\gap c\gap c\gap c\gap c\gap c\gap c\gap c\gap c\gap c\gap c\gap}
\includegraphics[width=\colwidth]{./images/splits_fashion/61_green_horse_093590446.png}&
\includegraphics[width=\colwidth]{./images/splits_fashion/24_green_car_0966971.png}&
\includegraphics[width=\colwidth]{./images/splits_fashion/74_green_bird_11749195.png}&
\includegraphics[width=\colwidth]{./images/splits_fashion/51_green_deer_11908391.png}&
\includegraphics[width=\colwidth]{./images/splits_fashion/91_green_cat_12119513.png}&
\includegraphics[width=\colwidth]{./images/splits_fashion/89_green_frog_1445258.png}&
\includegraphics[width=\colwidth]{./images/splits_fashion/12_green_horse_15427034.png}&
\includegraphics[width=\colwidth]{./images/splits_fashion/95_green_ship_16562095.png}&
\includegraphics[width=\colwidth]{./images/splits_fashion/26_green_frog_1981184.png}&
\includegraphics[width=\colwidth]{./images/splits_fashion/17_green_deer_20366296.png}&
\includegraphics[width=\colwidth]{./images/splits_fashion/23_red_truck_21338153.png}&
\includegraphics[width=\colwidth]{./images/splits_fashion/42_red_cat_2537753.png}&
\includegraphics[width=\colwidth]{./images/splits_fashion/25_red_deer_3678056.png}&
\includegraphics[width=\colwidth]{./images/splits_fashion/67_red_cat_6120715.png}&
\includegraphics[width=\colwidth]{./images/splits_fashion/68_red_truck_64.png}\\

0.094 &
0.097 &
0.117 &
0.119 &
0.121 &
0.145 &
0.154 &
0.166 &
0.198 &
0.204 &
0.213 &
0.254 &
0.368 &
0.612 &
0.64 \\

\end{tabular}
\caption{}
\label{}
\end{figure*}

==> latex/25_fig_cifar100strip.tex <==
\renewcommand{\colwidth}{ 0.060000000000000005 \linewidth}
\renewcommand{\gap}{@{\hspace{0.5mm}}}

\begin{figure*}
\centering

\begin{tabular}{c\gap c\gap c\gap c\gap c\gap c\gap c\gap c\gap c\gap c\gap c\gap c\gap c\gap c\gap c\gap}
\includegraphics[width=\colwidth]{../../split_images/06_green_76_1705506.png}&
\includegraphics[width=\colwidth]{../../split_images/07_green_16_20248191.png}&
\includegraphics[width=\colwidth]{../../split_images/56_green_71_20544866.png}&
\includegraphics[width=\colwidth]{../../split_images/33_green_24_20687903.png}&
\includegraphics[width=\colwidth]{../../split_images/66_green_43_20696922.png}&
\includegraphics[width=\colwidth]{../../split_images/96_green_50_73123133.png}&
\includegraphics[width=\colwidth]{../../split_images/51_green_22_7378193.png}&
\includegraphics[width=\colwidth]{../../split_images/93_green_44_7430873.png}&
\includegraphics[width=\colwidth]{../../split_images/58_green_06_8402666.png}&
\includegraphics[width=\colwidth]{../../split_images/98_green_07_84480155.png}&
\includegraphics[width=\colwidth]{../../split_images/29_red_46_76185423.png}&
\includegraphics[width=\colwidth]{../../split_images/01_red_83_7696611.png}&
\includegraphics[width=\colwidth]{../../split_images/03_red_91_7753155.png}&
\includegraphics[width=\colwidth]{../../split_images/91_red_11_8513227.png}&
\includegraphics[width=\colwidth]{../../split_images/29_red_70_86318165.png}\\

0.171 &
0.202 &
0.205 &
0.207 &
0.207 &
0.731 &
0.738 &
0.743 &
0.84 &
0.845 &
0.762 &
0.77 &
0.775 &
0.851 &
0.863 \\

\end{tabular}
\caption{}
\label{}
\end{figure*}
